UMIE: Unified Multimodal Information Extraction with Instruction Tuning

Multimodal information extraction (MIE) gains significant attention as the popularity of multimedia content increases. However, current MIE methods often resort to using task-specific model structures, which results in limited generalizability across tasks and underutilizes shared knowledge across MIE tasks. To address these issues, we propose UMIE, a unified multimodal information extractor to unify three MIE tasks as a generation problem using instruction tuning, being able to effectively extract both textual and visual mentions. Extensive experiments show that our single UMIE outperforms various state-of-the-art (SoTA) methods across six MIE datasets on three tasks. Furthermore, in-depth analysis demonstrates UMIE's strong generalization in the zero-shot setting, robustness to instruction variants, and interpretability. Our research serves as an initial step towards a unified MIE model and initiates the exploration into both instruction tuning and large language models within the MIE domain. Our code, data, and model are available at https://github.com/ZUCC-AI/UMIE

==> sections/performance-ace05.tex <==

\begin{table}[t]
\small
\centering

% \resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|c|c|cc} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
\toprule 
 \multirow{2}{*}{}&   \multirow{2}{*}{\textbf{NER}} & \multirow{2}{*}{\textbf{RE}} & \multicolumn{2}{c}{\textbf{EE}}\\

&   &   &  \multicolumn{1}{c}{Event} &\multicolumn{1}{c}{Arg.} \\

 \midrule
UIE-base   &85.8 & 66.1 & 73.36 & 54.79 \\
UMIE-base  &85.5 & 65.9 & 71.26 & 52.07 \\
    \bottomrule
\end{tabular}
\caption{Performance of  ACE05 in finetune  (\%). }\label{tab:result}
    % }	    
\end{table}

==> tables/rebuttal_instruction_prefix.tex <==
\begin{table}[tbh]
    \centering
    \small
    \resizebox{1.0\linewidth}{!}{

    \begin{tabular}{l|ccc|cc|cc} 
    \toprule 
    \multicolumn{1}{c|}{\multirow{3}{*}{\centering \textbf{Method}}} &  \multicolumn{3}{c}{\textbf{MNER}} & \multicolumn{2}{c}{\textbf{MRE}} & \multicolumn{2}{c}{\textbf{MEE}} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}

    &  \multicolumn{1}{c}{T-15} & \multicolumn{1}{c}{T-17}  & \multicolumn{1}{c}{SNAP}  & \multicolumn{1}{|c}{RE-V1} &\multicolumn{1}{c|}{RE-V2} & \multicolumn{1}{c}{MED} &\multicolumn{1}{c}{MEAE} \\
     \midrule
Base (w/ IP)  &  76.3  & 91.7 & 91.0 & 84.2 & 76.0 & 60.6 & 23.1 \\
Base (w/o IP) & $74.9_{\blue{-1.4}}$ & $89.7_{\blue{-2.0}}$ & $89.4_{\blue{-1.6}}$ & $83.7_{\blue{-0.5}}$ & $74.3_{\blue{-1.7}}$ & $59.7_{\blue{-0.9}}$ & $22.5_{\blue{-0.6}}$\\ 
\midrule
Large (w/ IP)  &  77.3 & 92.0  & 91.3  & 86.7 & 77.6 &62.0 & 24.2\\ 
Large (w/o IP) & $76.0_{\blue{-1.3}}$  & $90.1_{\blue{-1.9}}$ & $90.3_{\blue{-1.0}}$ & $84.6_{\blue{-2.1}}$ & $75.4_{\blue{-2.2}}$ & $60.2_{\blue{-1.8}}$ & $23.3_{\blue{-0.9}}$ \\
\midrule
XLarge (w/ IP) & 78.4 & 93.1  & 91.8 & 87.2 & 78.3 &62.5 & 24.9\\
XLarge (w/o IP) & $77.3_{\blue{-1.1}}$  & $91.0_{\blue{-2.1}}$ & $90.5_{\blue{-1.3}}$ & $86.7_{\blue{-0.5}}$ & $76.2_{\blue{-2.1}}$ & $60.9_{\blue{-1.4}}$ & $24.1_{\blue{-0.8}}$ \\
% \midrule
       \bottomrule
    \end{tabular}

}
        \caption{Performance of UMIE with (w/) and without (w/o) instruction prefix (IP).}
        \label{tab:result-no-instruction}
\vspace{-1em}
\end{table}

==> tables/rebuttal_twitter15.tex <==
\begin{table}[t]
\centering
  \resizebox{1.0\linewidth}{!}{
\small
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\textbf{Method} & \textbf{UMT} & \textbf{CAT-MNER} & \textbf{BGA-MNER}  & \textbf{Base} & \textbf{Large} &  \textbf{XLarge}\\
\midrule
Twitter-15 & 64.1 & 68.4 & 68.7  &  66.9 & 68.3  & \textbf{69.1}\\
\bottomrule
\end{tabular}
}
\caption{Performance on zero-shot Twitter-15. Base, Large, and XLarge are UMIE models with different sizes.}
\label{tab:zero-shot-t15}
\vspace{-1em}
\end{table}


==> tables/text_only.tex <==
\begin{table}[t]
\centering
    % \resizebox{0.5\linewidth}{!}{
    \small
    \centering
    \begin{tabular}{l|c}
    \toprule
    \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{}}} &  \multicolumn{1}{c}{UMIE-large}  \\
    \midrule
   Twitter-15 &77.5\\
   Twitter-17 & 92.1 \\
   SNAP  & 91.5\\
   MNER-V1& 83.9\\
   MNER-V2& 76.1\\
   M$^2$E$^2$ MED & 62.6  \\
   M$^2$E$^2$ MEAE & 25.4  \\
 \bottomrule
    \end{tabular}
     \caption{Performance of text-only in UMIE-large (\%).}     \label{tab:text-only}
 
    % }	
\end{table}
